Gen-Oja: A Two-time-scale approach for Streaming CCA

In this paper, we study the problems of principal Generalized Eigenvector computation and Canonical Correlation Analysis in the stochastic setting. We propose a simple and efficient algorithm, Gen-Oja, for these problems. We prove the global convergence of our algorithm, borrowing ideas from the theory of fast-mixing Markov chains and two-time-scale stochastic approximation, showing that it achieves the optimal rate of convergence. In the process, we develop tools for understanding stochastic processes with Markovian noise which might be of independent interest.

==> bak.tex <==
\begin{itemize}
\item Problem statement: what are we studying and which is the problem 
\item our apporach: we present our algorithm and give some intuition. we also briefly explain how we study the markovian noise which is the main difference with usual stochastic approximation.
\item result: present and comment our result. sketch of the proof: how we transform the problem to a matrix operator.
\item Application to CCA
\end{itemize}

%Let us assume we observe a stream of matrices $A_1,\dots,A_t\in \R^{d\times d}$ and $B_1,\dots,B_t\in \R^{d\times d}$ assumed to be drawn i.i.d. from an unknown underlying distribution, such that $\E[A_i]=A$ and $\E[B_i]=B$ where $A$ is a symmetric matrix and $B$ is symmetric positive definite matrix and we want to compute the principal generalized eigenvector of $(A,B)$ which is defined as the maximizer of the generalized Rayleigh quotient:
%\begin{equation}\label{eq:geneigen}
%v_1= \arg \max_{v\in\R^d} \frac{ v^\top A v }{v^\top B v}.
%\end{equation}


For a symmetric  positive semidefinite matrix $M$, we let $\Vert v\Vert_M=\sqrt{v^\top M v}$ denote the $M$-norm of $u$ and define similarly the inner product of $u$ and $v$ in the $M$-norm as $\langle u,v\rangle_M=u^\top M v$. \note{check if we use it}  
We specifically denote by $\lambda_1,\dots, \lambda_2$ the eigenvalues of $B^{-1}A$ (which exists thanks to Lemma ), satisfying $\lambda_1>\dots > \lambda_d$ and $(v_i)_{i=1\dots d}$ and $(\tilde v_i)_{i=1\dots d}$ the corresponding right and left eigenvector. In order to quantify the error between vectors we define the sinus in the $B$ norm between two vectors as 
\[
\sin_B(v,w)= 1-\Big(\frac{v^\top B w}{\Vert V \Vert_B\Vert w \Vert_B}\Big)^2.
\]
We will see above it is important for us to work in the $B$-norm. The other quantities of interest are the eigengap $\delta =\lambda_1-\lambda_2$ and the condition number of the matrix $B$,  $\kappa= \frac{\lambda_{\max}(B)}{\lambda_{\min}(B)}$. We also assume that 
\[ \Vert A_t\Vert \leq R_A  \quad \text{ and } \quad \Vert B_t\Vert \leq R_B \quad \text{ almost surely}
\]

%In the offline setting, given access to $A$ and $B$, \cite{ge2016} recently proposed to solve this problem using an approximate power method on $B^{-1}A$, where in each iteration, they proposed to solve the least squares problem $\min_{w\in \R^d} \Vert B^{1/2} w - A v_t\Vert_2^2$ using fast linear system solvers. This leads to the following nested-loop approach: an outer loop for performing approximate power method and an inner loop for performing least squares regression. 

%A natural extension of the nested-loop approach in the stochastic setting would be to use  batches of samples for solving the least squares problem and performing a noisy power method step. 

%Consider the setting where we observe an online sequence of matrices  where $A$ is a symmetric matrix and $B$ is symmetric positive definite matrix. The principle generalized eigenvector $v_1$, of the system $(A, B)$ corresponds to the 
%This is equivalently the eigenvector corresponding to the largest eigenvalue of $B^{-1}A$\footnote{We are computing the eigenvalue corresponding to the largest eigenvalue whereas other works focus on the largest eigenvalue in absolute value. However we can still solve the problem for $-A$ and consider the maximum of both.}. It is worth noted it is also closely related to the principal eigenvector of the symmetric matrix $B^{-1/2}AB^{-1/2}$. In this sense, this amount in doing the PCA of $A$ in the $B$ norm. If we had access to $A$ and $B$, directly solving this method would be computationally to expensive but we could approximately solve it by doing the power method (or a more involve algorithm as the Lanczos method) to either $B^{-1/2}AB^{-1/2}$ or $B^{-1}A$ which still needs to compute the inverse of these matrices.  Previous works proposed to approximate one step of power method $B^{-1}Av_t$ by solving the least square problem $\min_{w\in \R^d} \Vert B^{1/2} w - A v_t\Vert_2^2$, resulting in algorithm in two-steps: a inner loop approximating the solution of the Least-Squares and an outer loop computing the power-method updates. However we only have access to unbiased estimates of these matrix and these methods are inherently off-line. If it is still possible to collect samples and construct estimates $\hat A$ and $\hat B$ of these matrices,  they do not leverage the power of obtaining fresh samples $A_t,B_t$ at each step.  

We propose a new purely online algorithm to solve the problem in \eq{geneigen} which is describe in \myalgo{SPGE}. We iteratively update two sequence $(w_t,v_t)$: $w_t$ is updated as one step of stochastic gradient descent with constant step-size to minimize $ \Vert B^{1/2} w- A v_{t-1}\Vert_2^2$ (using the gradient estimate $B_tw-Av_{t-1}$) and $v_t$ is updated as one step of Oja algorithm taking $w_t v_{t-1}^\top$ as noisy matrix. This algorithm takes its roots in the two time-scale approximation framework.

